Fire!

In this paper, we provide an epistemic analysis of a simple variant of the fundamental consistent broadcasting primitive for byzantine fault-tolerant asynchronous distributed systems. Our Firing Rebels with Relay (FRR) primitive enables agents with a local preference for acting/not acting to trigger an action (FIRE) at all correct agents, in an all-or-nothing fashion. By using the epistemic reasoning framework for byzantine multi-agent systems introduced in our TARK'19 paper, we develop the necessary and sufficient state of knowledge that needs to be acquired by the agents in order to FIRE. It involves eventual common hope (a modality related to belief), which we show to be attained already by achieving eventual mutual hope in the case of FRR. We also identify subtle variations of the necessary and sufficient state of knowledge for FRR for different assumptions on the local preferences.

==> eptcsdata.tex <==
\providecommand{\firstpage}{139}
\providecommand{\publicationstatus}{J. Y. Halpern and A. Perea (Eds.): Theoretical Aspects \\
of Rationality and Knowledge 2021 (TARK 2021) \\
EPTCS 335, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.335.13}{10.4204/EPTCS.335.13}}

